SLUE: New Benchmark Tasks for Spoken Language Understanding Evaluation on Natural Speech

Progress in speech processing has been facilitated by shared datasets and benchmarks. Historically these have focused on automatic speech recognition (ASR), speaker identification, or other lower-level tasks. Interest has been growing in higher-level spoken language understanding tasks, including using end-to-end models, but there are fewer annotated datasets for such tasks. At the same time, recent work shows the possibility of pre-training generic representations and then fine-tuning for several tasks using relatively little labeled data. We propose to create a suite of benchmark tasks for Spoken Language Understanding Evaluation (SLUE) consisting of limited-size labeled training sets and corresponding evaluation sets. This resource would allow the research community to track progress, evaluate pre-trained representations for higher-level tasks, and study open questions such as the utility of pipeline versus end-to-end approaches. We present the first phase of the SLUE benchmark suite, consisting of named entity recognition, sentiment analysis, and ASR on the corresponding datasets. We focus on naturally produced (not read or synthesized) speech, and freely available datasets. We provide new transcriptions and annotations on subsets of the VoxCeleb and VoxPopuli datasets, evaluation metrics and results for baseline models, and an open-source toolkit to reproduce the baselines and evaluate new models.

==> figures_and_tables.tex <==
\section{tables}










% \begin{table}[]
% \centering
% \resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sentiment\\ Label\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Sets\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Human Perf.\\($F_1$ on Test)\end{tabular}} \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}l@{}}Finetune\end{tabular} & \begin{tabular}[c]{@{}l@{}}Dev\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test\end{tabular} & Audio   & Text \\ \hline
% Negative & 227 & 3 & 204 & 0.39 & 0.5\\ \hline\textbf{}
% Neutral & 4,223 & 784 & 2,770 & 0.82 & 0.84\\ \hline
% Positive & 1,279 & 167 & 929 & 0.67 & 0.64\\ \hline
% Mixed & 48 & 1 & 30 & - & -\\ \hline
% Disagreement & - & - & 119 & - & -\\ \hline \hline
% Total & 5,777 & 955 & 4,052 & - & -\\ \hline
% \end{tabular}%
% }
% \caption{Voxceleb Sentiment label statistics. Sentiments Spearman's rank correlation coefficient (as a measure of inter-annotator agreement) for passes $P_1$, $P_2$, and $P_3$:
% $P_1 \text{ vs }P_2 = 0.49$, $P_2 \text{ vs } P_3 = 0.39$, $P_1 \text{ vs } P_3 = 0.38$. Fleiss' Kappa score: $\kappa=0.33$.}
% \label{voxceleb_stats}
% \end{table}
% \begin{table}[]
% \centering
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{c|ccc}
% \hlineB{2}
% \multirow{2}{*}{Sentiment label} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Sets\end{tabular}}  \\ \cline{2-4} 
%  & \begin{tabular}[c]{@{}l@{}}Finetune\end{tabular} & \begin{tabular}[c]{@{}l@{}}Dev\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test\end{tabular} \\ \hline
% Negative & 227 & 3 & 204 \\ 
% Neutral & 4,223 & 784 & 2,770 \\ 
% Positive & 1,279 & 167 & 929 \\ 
% Mixed & 48 & 1 & 30 \\ \
% Disagreement & - & - & 119 \\ \hline \hline
% Total & 5,777 & 955 & 4,052 \\ \hlineB{2}
% \end{tabular}%
% }
% \caption{Voxceleb Sentiment label distribution.}
% \label{tab:voxceleb_stats}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/fourth_pass_audio.png}
%     \caption{Reference labels vs held-out pass. \\F1 scores: Negative (0.39), Neutral (0.82), Positive (0.67)}
%     \label{fig:pass_audio}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/fourth_pass_text.png}
%     \caption{Reference labels vs text-only held-out pass. \\F1 scores: Negative (0.50), Neutral (0.84), Positive (0.64)}
%     \label{fig:pass_text}
% \end{figure}


% \begin{table}[]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Dev} & \multicolumn{2}{c|}{Test} \\ \cline{2-5} 
% \multicolumn{1}{|c|}{} & Unweighted & Weigthed & Unweighted & Weighted \\ \hline
% \textbf{NLP Topline} : & & & & \\ 
% \hspace{2mm} GT Text + BERT-base &  &  &  &  \\ 
% \hspace{2mm} GT Text + DeBERTa-base &  &  &  &  \\ 
% \hspace{2mm} GT Text + DeBERTa-large &  &  &  &  \\ \hline
% \textbf{Pipeline approaches} : & & & & \\ 
% \hspace{2mm} W2V2-base + DeBERTa-large &  &  &  &  \\ 
% \hspace{2mm} W2V2-large-LL60K + DeBERTa-large &  &  &  &  \\
% \hspace{2mm} W2V2-base (+LM) + DeBERTa-large &  &  &  &  \\ 
% \hspace{2mm} W2V2-large-LL60K (+LM) + DeBERTa-large &  &  &  &  \\ \hline
% \textbf{E2E approaches} : & & & & \\ 
% \hspace{2mm} W2V2-base &  &  &  &  \\ 
% \hspace{2mm} W2V2-base-VP100K &  &  &  &  \\ 
% \hspace{2mm} HuBERT-base &  &  &  &  \\ 
% \hspace{2mm} W2V2-large-LL60K &  &  &  &  \\ \hline
% \end{tabular}%
% }
% \caption{NER detail performance (F1) \suwon{Why don't we drop label-f1 score here?}
% \label{tab:ner_detail}\ap{I think we can skip fscore-label, but add a line about it in the text -- follows the same trend, typically a few (quantify) points higher than fscore}\ap{can we skip base/large suffixes with B and L? It'll make column 1s smaller for all tables.}\ap{Any specific reason to not have BERT-base and DeBERTa-base models for the Pipeline variants (given that we have those for NLP variants?)}}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multicolumn{3}{|c|}{Model}       & \multicolumn{2}{c|}{Dev} & \multicolumn{2}{c|}{Test} \\ \hline
% \multicolumn{1}{|c|}{Speech model}  & LM   & Text model   & Unweighted  & Weighted  & Unweighted   & Weighted  \\ \hline
% \textbf{NLP Toplines:}  &  & & &  &  &  \\
% \hspace{12mm} \multirow{3}{*}{\normalsize N/A} & \multirow{3}{*}{\normalsize N/A}  & BERT-B & &  &  &  \\
% % \multicolumn{2}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}N/A\\ (NLP topline)\end{tabular}}}  & BERT-base & &  &  &  \\
% &  &  DeBERTa-B & &  &  &  \\
% & & DeBERTa-L   & &  &  &  \\ \hline
% \textbf{Pipeline approaches:}  &  &  &  &  & & \\
% \hspace{2mm} W2V2-B  & - & BERT-B & &  &  &  \\
% \hspace{2mm} W2V2-B  & - & DeBERTa-B & &  &  &  \\
% \hspace{2mm} W2V2-B  & - & DeBERTa-L & &  &  &  \\
% \hspace{2mm} W2V2-L-LL60K &  -   &  DeBERTa-L   & &  &  &  \\ \hline
% \hspace{2mm} W2V2-B  &  \cmark  &  BERT-B   & &  &  &  \\
% \hspace{2mm} W2V2-B  &  \cmark  & DeBERTa-B   & &  &  &  \\
% \hspace{2mm} W2V2-B  &  \cmark  & DeBERTa-L   & &  &  &  \\
% \hspace{2mm} W2V2-L-LL60K &  \cmark &  DeBERTa-L  & &  &  &  \\ \hline
% \textbf{E2E approaches:}  &  &  &  &  & & \\
% \hspace{2mm} W2V2-B  & - & \multirow{4}{*}{\normalsize N/A} &  &  &  &  \\
% \hspace{2mm} W2V2-B-VP100K &  -  &  & &  &  &  \\
% \hspace{2mm} HuBERT-B &  -   &   & &  &  &  \\
% \hspace{2mm} W2V2-L-LL60K &  - &    & &  &  &  \\ \hline
% \hspace{2mm} W2V2-B & \cmark & \multirow{4}{*}{\normalsize N/A} & &  &  &  \\ 
% \hspace{2mm} W2V2-B-VP100K  & \cmark &    & &  &  &  \\
% \hspace{2mm} HuBERT-B  &  \cmark   &    & &  &  &  \\
% \hspace{2mm} W2V2-L-LL60K & \cmark  &  & &  &  &   \\ \hline
% \end{tabular}}
% \caption{NER performance (F-score)\ap{wip}
% % \ap{Thoughts on this alternate table representation? I separated the model name out in three columns so that it's easier to parse. I did like the explicit mentions of {\bf NLP Topline}, etc. in the previous table which I find tricky to include here.} 
% % \suwon{how about this? we may need to unify the table form for all baselines}
% % \kl{I like it. very minor suggestion for the LM column:  leave it empty instead of the "x" to indicate no LM (the checks and Xs are not that different from a distance, and the tables are very dense already)}
% % \ap{Any specific reason to not have BERT-base and DeBERTa-base models for the Pipeline variants (given that we have those for NLP variants?)}
% % \suwon{ I think we talked about just leave the best nlp model after NLP topline experiment. The combination in the pipeline is also still odd to me. why no w2v2-b + deberta-L?}
% % \ap{Yes that's valid too, added it. I think this table as a more exhaustive version of table 7. I'll just add all the numbers for now, we can then choose to remove some later.}
% % \suwon{Yep. I also have all number in these combination, but the trend is the same like in NLP topline, so it's predictable. maybe we can put all this still if we have space, but we can also mention briefly if we don't have enough space. Feel free to make these comments invisible if you already reflected and solved!}
% }
% \label{tab:ner_task_detail}
% \end{table}




% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|c|c|c|c|c}
% \hline
% \multirow{3}{*}{Type} & \multirow{3}{*}{Used pre-trained model} & \multicolumn{3}{c|}{ASR} & NER & SA \\ \cline{3-7}
% & & \multicolumn{3}{|c|}{WER (\st{WER with LM}) $\downarrow$} & F1 / label-F1 ( +LM ) $\uparrow$ & Acc / F1 (weighted acc / F1) $\uparrow$ \\ \cline{3-7}
% &  & (Librispeech) & Voxpopuli & Voxceleb & Voxpopuli & Voxceleb \\ \hline
% % \multicolumn{6}{c}{\st{Human performance}} \\ \hline
% %  & - / 5.83~\cite{amodei2016deep} & - / - & - / - &  &  \\ \hline
% % \multicolumn{6}{c}{\st{Supervised Baseline (without unsupervised pre-trained model})} \\
% % \hline
% % \st{MFCC/Fbank+LSTM/CNN} & - (-) & - (-) & - (-) & - (-) & 32.9 / 30.2 (66.7 / 59.1) \\
% % \multicolumn{6}{c}{Pipeline Topline (Ground Truth Text + NLP Models)} \\ \hline
% % GT Text + BERT-base & - (-) & - (-) & - (-) & - (-) & 54.1 / 56.2 (78.6 / 77.2) \\
% % GT Text + DeBERTa-base & - (-) & - (-) & - (-) & - (-) & 56.8 / 58.9 (78.4 / 77.5) \\
% % \hline
% % \multicolumn{6}{c}{Pipeline Baseline (ASR + NLP Models)} \\
% % \hline
% % W2V2-base-LS960 ASR (+LM) + BERT-base & - (-) & - (-) & 20.5 (15.8) & - (-) & - / - (- / -) \\
% % W2v2-large-LL60K ASR (+LM) + DeBERTa-large & - (-) & - (-) & 15.6 (12.0) & - (-) & - / - (- / -) \\
% % \hline
% % \multicolumn{6}{c}{E2E Baselines} \\
% % \hline
% % W2V2-base-LS960 & - (-) & - (-) & 20.5 (15.8) & - (-) & - / - (- / -) \\
% % W2V2-base-VP100K & - (-) & - (-) & 33.4 (22.6) & - (-) & - / - (- / -) \\
% % HuBERT-base-LS960 & - (-) & - (-) & 21.2 (16.1) & - (-) & - / - (- / -) \\
% % W2V2-large-LL60K & - (-) & - (-) & 15.6 (12.0) & - (-) & - / - (- / -) \\


% % \multirow{1}{*}{ \st{Supervised} }
% %  & MFCC+LSTM/CNN & - (-) & - (-) & - (-) & - / - (- / -) & 32.9 / 30.2 (66.7 / 59.1) \\
% \hline
% \multirow{1}{*}{ NLP topline }
% %  & GT Text + BERT-base & - (-) & - (-) & - (-) & - / - (- / -) & 54.1 / 56.2 (78.6 / 77.2) \\
% %  & GT Text + DeBERTa-\textbf{base} & - (-) & - (-) & - (-) & - / - (- / -) & 56.8 / 58.9 (78.4 / 77.5) \\
%  & GT Text + DeBERTa-large & - (-) & - (-) & - (-) & - / - (- / -) & 56.8 / 58.9 (78.4 / 77.5) \\
% \hline
% \multirow{1}{*}{ Pipeline }
% %  & \st{W2V2-base ASR (+LM) + BERT-base} & 17.6 (9.5) & 17.2 (14.3) & 20.5 (15.8) & - / - (- / -) & - / - (- / -) \\
% %  & W2V2-base (+LM) + DeBERTa-base & 9.5 & 14.3 & 15.8 & - / - (- / -) & - / - (- / -) \\
%  & W2V2-large-LL60K (+LM) + DeBERTa-large & 5.8 & - & 12.0 & - / - (- / -) & - / - (- / -) \\
% \hline
% \multirow{4}{*}{ E2E }
%  & W2V2-base & 17.6 & 17.2 & 20.5 & - / - (- / -) & - / - (- / -) \\
%  & W2V2-base-VP100K & - & 21.6  & 33.4  & - / - (- / -) & - / - (- / -) \\
%  & HuBERT-base & -  & 18.6  & 21.2  & - / - (- / -) & - / - (- / -) \\
%  & W2V2-large-LL60K & 10.0 & -  & 15.6 & - / - (- / -) & - / - (- / -) \\
%  \hline
% %  \multirow{4}{*}{ E2E + LM}
% %  & W2V2-base & 17.6 (9.5) & 17.2 (14.3) & 20.5 (15.8) & - / - (- / -) & - / - (- / -) \\
% %  & W2V2-base-VP100K & - (-) & 21.6 (16.5) & 33.4 (22.6) & - / - (- / -) & - / - (- / -) \\
% %  & HuBERT-base & - (9.4) & 18.6 (15.4) & 21.2 (16.1) & - / - (- / -) & - / - (- / -) \\
% %  & W2V2-large-LL60K & 10.0 (5.8) & - (-) & 15.6 (12.0) & - / - (- / -) & - / - (- / -) \\
% % \hline
% \end{tabular}%
% }
% \caption{baseline performance for slue benchmark}
% \label{performance}
% \end{table*}





